FastScan: Robust Low-Complexity Rate Adaptation Algorithm for Video Streaming over HTTP

This paper proposes and evaluates a novel algorithm for streaming video over HTTP. The problem is formulated as a non-convex optimization problem which is constrained by the predicted available bandwidth, chunk deadlines, available video rates, and buffer occupancy. The objective is to optimize a QoE metric that maintains a tradeoff between maximizing the playback rate of every chunk and ensuring fairness among different chunks for the minimum re-buffering time. We propose FastScan, a low complexity algorithm that solves the problem. Online adaptations for dynamic bandwidth environments are proposed with imperfect available bandwidth prediction. Results of experiments driven by Variable Bit Rate (VBR) encoded video, video platform system (dash.js), and cellular bandwidth traces of a public dataset reveal the robustness of the online version of FastScan algorithm and demonstrate its significant performance improvement as compared to the considered state-of-the-art video streaming algorithms. For example, on an experiment conducted over 100 real cellular available bandwidth traces of a public dataset that spans different available bandwidth regimes, our proposed algorithm (FastScan) achieves the minimum re-buffering (stall) time and the maximum average playback rate in every single trace as compared to Bola, Festive, BBA, RB, and FastMPC, and Pensieve algorithms.

==> avcAlgo.tex <==
\section{Proposed Algorithm}

\begin{figure}[h]
		%\vspace{-.6in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
			\STATE {\bf Input:} ; $X_n(i)$, $s$, $B_m$, $C$, $B(j)$, 
			\STATE {\bf Output:} $X(i) \forall i$: The maximum size in which chunk $i$ can be fetched, $I_n$: set contains the indices of the chunks that can be fetched up to $n$th quality level.
					
    \STATE {\bf Initilization:}
    \STATE $X(i)=0$, $d(i)=0$, $deadline(i)=(i-1)L+s+d(i)$, $\forall i$
   \STATE $c(j)=\sum_{j^\prime=1}^{j}B(j^\prime)$ available bandwidth up to time $j$, $\forall j$
   \STATE $bf(j)=0$: buffer length at time $j$
   \STATE $t(i)=0, \forall i$, first time slot chunk $i$ can be fetched
   %\STATE $a(i)=0, \forall i$, lower layer decision of fetched amount of chunk $i$ at its lower deadline time $t(i)$
   \STATE $e(j)=B(j), \forall j$,  remaining  bandwidth at time j after all non skipped chunk are fetched %according to lower layer size decisions 
   \STATE {\bf Lowest Quality level decision, $n=0$:}
    \STATE $d=$ {\bf level-0-Forward}$(B, X, i^\prime, C,d, deadline,$ $B_m, bf, j^\prime)$
    \STATE $deadline(i)=(i-1)L+s+d(C)$
     \STATE $d={\bf level-0-Backward}(B, X_0, x, i^\prime, C, d,$ $deadline, B_m, bf, j^\prime)$
      \STATE $deadline(i)=(i-1)L+s+d(i)$
  \STATE {\bf Enhancement layer decisions:}
   \STATE {\bf For every enhancement layer $n$}
   \STATE $[t,a,e] =$ {\bf level-n-forward}$(B, X, i^\prime,C, deadline, B_m,bf,j^\prime, I_0)$
  \STATE $[X, I_n]=$ {\bf level-n-backward}$(B, X,X_{n}, i^\prime,C, L, deadline,$ $B_m,bf,j^\prime,t,c,a,e)$
   				\end{algorithmic}
				\caption{Deadline Aware Bin Packing Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}

We now describe our algorithm. ``Deadline and Buffer Aware Bin Packing Algorithm", which is summarized in Algorithm 1. At a high level,
our algorithm works from the lowest to the highest quality level, and processes each quality level for the chunks that are candidates for the previous one. The algorithm performs forward and backward scans (explained bellow) in sequence starting from the lowest quality level ({\bf level-0})(lines 7-9, and 13-14). %we described is ``{\em No-Skip Deadline and Buffer Aware Bin Packing Algorithm}" (Algorithm 5). An example run of the algorithm is described in Appendix \ref{noskipex}.
\begin{figure}[hbtp]
		%\vspace{-.6in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Output:} $d(i)$: stall time of chunk $i$.

 \STATE $ j=j^\prime$, $i=i^\prime$
    \WHILE {chunk $C$ is not fetched yet}
      		\IF{$(i > 1$ and $d(i) < d(i-1))$}
			\STATE $d(i)=d(i-1)$, $deadline(i)=(i-1)L+s+d(i)$
		\ENDIF
		\STATE{\bf if} $(bf(j) = Bm)$, {\bf then} $j=j+1$
                 \STATE $fetched=min(B(j), X(i))$
                 \STATE $B(j)=B(j)-fetched$, $X(i)=X(i)-fetched$
                 \STATE {\bf IF} $X(i) > 0$, {\bf then} $bf(j)=bf(j)+L$
                 \IF{$X(i)=0$ and $j <= deadline(i)$}
                      \STATE i=i+1
                \ELSIF{$X(i)=0$ and $j >deadline(i) $}
                \STATE $d(i)=d(i)+j-deadline(i)$
                     % \STATE $bf(t(i):deadline(i))=bf(t(i):deadline(i))+L$
                      \STATE $i=i+1$
                \ENDIF

                 \STATE {\bf if} $B(j)=0$, {\bf then} $j=j+1$
                   
                      \ENDWHILE

				\end{algorithmic}
				\caption{{\bf Level-0} Forward Algorithm}
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}
	
	
	\begin{figure}[hbtp]
		%\vspace{-.6in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
					\STATE {\bf Output:} $d_f(i)$: final stall duration of chunk $i$.
					
    \STATE {\bf Initilization:}
    \STATE $i=C$, $ j=deadline(C)$

     \WHILE {($j >( j^\prime-1)$ and $i > (i^\prime-1)$)}
     \IF{$(i < C)$}
     	\STATE $d_f(i)=d(i)-(d(i-1)-d_f(i-1))$ 
	\STATE $deadline(i)=(i-1)L+s+d_f(i)$
     \ENDIF
        \IF{$j <= deadline(i)$}
        			\STATE {\bf if}($bf(deadline(i)) = B_m)$, {\bf then} $d_f(i)=d(i)-1$
               		
               		\STATE $fetched=min(B(j),X_0(i))$
               		\STATE $X_0(i)=X_0(i)+fetched$, $B(j)=B(j)-fetched$
                 	\STATE {\bf if}$(X(i) > 0)$, {\bf then} $bf(j)=bf(j)+L$
                		\STATE {\bf if}$(X_0(i) = 0)$, {\bf then} $i=i-1$
                	 	\STATE {\bf if}$(B(j) = 0)$, {\bf then} $j=j-1$
           \ELSE
           	\STATE $j=j-1$
        \ENDIF
\ENDWHILE

				\end{algorithmic}
				\caption{{\bf Level-0} Backward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}


{\bf level-0 Forward scan}: Given the predicted bandwidth the buffer size, and the prediction window size $W$, the algorithm simulates fetching next $W$ chunks at lowest quality level and determines the minimum stall duration of this segment since that is the first priority.  Let's assume that the current $W$ chunks are the chunks from $i^\prime$ to $C$ where $C=i^\prime+W-1$. The algorithm simulates fetching these chunks in order at the lowest quality level (Algorithm 2) with an assumption that the stall time is zero. i.e, $d(i^\prime)=\cdots = d(C)=0$. Therefore, the initial deadline of every chunk $i$ such that $i^\prime \leq i \leq C$ is $(i-1)L+s$. Where $s$ is the startup delay plus all stalls before $i^\prime$ (i.e $s$ is the total stall duration before the current segment. Chunks are fetched in order and if a chunk $i$ can't be completely downloaded before violating its initial deadline, the additional time spent in fetching this chunk is added to $d(i^{\prime\prime})$ for every $i \leq i^{\prime\prime} \leq C$ since there has to be an additional stall in order to fetch these chunks (line 22-25). Therefore, this forward scan finds the stall duration and the deadline of the last chunk ($d(C)$, and $deadline(C)$) such that all chunks are guaranteed to be fetched at least at the lowest quality level. Finally, {\bf level-0 Forward scan} is repeated after the download of every chunk.

{\bf level-0 Backward scan}: One thing to note from the results of the forward scan. forward scan gives a guarantee that all chunks from $i^\prime$ to $C$ can be fetched at least at lowest quality level with minimum stall duration when the deadline of the last chunk $C$ is set to $deadline(C)$ that was found by forward scan. However, stalls could still occur in the middle of the segment which means more number of video interruptions (less smoothness) and less opportunity to fetch later chunks at higher quality levels. Therefore,  {\bf level-0 Backward scan} is run after that to push all stalls if possible (i.e if buffer allows) to the beginning of the segment (before chunk $i^\prime$. Given the predicted bandwidth, the forward scan decisions and the buffer size, (Algorithm 3) simulates fetching chunks at {\bf level-0} quality starting from the last toward the first chunk (lines 4-6). The backward algorithm objective is to move stalls to their earliest time. i.e, as early as possible. In fact if the buffer is infinite, all stalls can be brought to the beginning of the current segment, but if the buffer is finite, that may not be always possible. {\bf Level-0} backward algorithm simulates fetching chunks in reverse order starting at the deadline of the last chunk ($j=deadline(C)= (C-1)L+s+d(C)$), and there will be one scenario that leads to changing the initial deadline and having a stall that is not brought to the very beginning of the current prediction period which is the buffer constraint violation (lines 12-15). If fetching a chunk $i$ results in a buffer constraint violation, the algorithm decrements the deadline of chunk $i$ by 1 and checks if the violations can be removed. This decrement can be continued till the violations are avoided. This provides the deadlines of the different chunks such that stall duration is at its minimum and stalls are brought to their earliest possible time. i.e minimum number of stalls and optimal stall pattern are found. When stalls are brought to their earliest possible, all chunks can have more time to increase their qualities without violating $deadline(C)$. Therefore, later chunks have higher chance of increasing their quality.

Once {\bf level-0} decisions are found, {\bf level-n} forward, and {\bf level-n} backward algorithms (Algorithm 4, and 5) are run per level. The key difference of {\bf level-n}  forward and {\bf level-n} backward scans with compare to {\bf level-0}  forward and backward scans is that the deadlines are fixed and can't be changed. 

{\bf level-n} forward algorithm simulates fetching chunks in order, where chunks are fetched according to $(n-1)$th level decision. The main objective of {\bf level-n} forward algorithm is to determine the lower deadline of every chunk $i$ in which chunk $i$ can't be fetched earlier ($t(i)$); otherwise, lower level decisions become violated. As we will see next, the lower and upper deadlines of every chunk are the key components that {\bf level-n} backward algorithm use to make a decision which chunk can be fetched at $n$th quality level.

% such that the number of chunks fetched at $n$th quality level is maximized without violating the lower quality level decisions. i.e. {\bf level-n} forward algorithm finds the chunks that can be posted to next quality level without creating un-necessary and more than one quality level switching between neighboring chunks preserves the smoothness of the quality level 

%with one change which is assuming that chunks that were candidates to $(n-1)$th quality level are fetched at $n$th quality level. i.e. $n$th level is considered only for chunks that were candidates for $(n-1)$th quality level

{\bf level-n} backward algorithm takes as input the lower and the upper deadlines of every chunk and finds which chunks can be pushed to the $n$th quality level. If pushing a chunk to $n$th quality level is not possible without violating its lower and upper deadlines, the chunk will not be candidate to $n$th quality level. i.e $Z_{n,i}=0$. \textit{Therefore, we clearly see that the algorithm prioritize pushing the maximum number of chunks to $n-1$ quality level over fetching some at $n$th quality level with the cost of reducing the quality of some others bellow $n-1$th quality level. This will prioritize horizontal over vertical scanning which reduces the quality switching that spanning more than one level.}
%{\bf level-n Forward algorithm}: (Algorithm 3) is run to simulate fetching chunks in order with quality decisions up to $(n-1)$th level and provides lower deadlines of chunks for the level-n backward run. Then, forward  scan finds the lower deadline of every chunk, so the lower level decisions are not violated.

 Running backward scan at $n$th level is the most tricky part since $Z_{n,i}$ for $n > 0$ can be zero. Given the predicted bandwidth, the lower and upper deadline of every chunk, and the buffer size, the algorithm simulates fetching the chunks in reverse order. The algorithm increases the size of every chunk that was a candidate to $(n-1)$ to $n$th quality level size. For every chunk $i$, the backward algorithm checks the bandwidth and the buffer; if there is enough bandwidth and the buffer is not full, then chunk $i$ is selected to be fetched at $n$th quality level (line 18-22). If a chunk $i^\prime$ that was a candidate to $(n-1)$th quality level is not selected to be fetched at $n$th quality level, one of the two scenarios could have happened. The first is the violation of {\bf buffer} capacity, where the chunk could not be placed in the buffer before its deadline (line 8). The second is the {\bf bandwidth} constraint where the remaining available bandwidth is not enough for fetching the chunk at $n$th quality level size (lines 15-17). This scenario also means that the chunk could not be fetched by the deadline, so it can also be called deadline violation.

For buffer capacity violation, we first note that, there could be a chunk  $i^{\prime\prime} > i^\prime$ in which if it was not fetched at $n$th quality level, chunk $i^{\prime}$ could have been $n$th level candidate. However, the {\bf level-n}  backward algorithm decides to not consider $i^\prime$ (line 8). We note that since there is a buffer capacity violation, one of the chunks must be skipped (not considered for $n$th level). The reason of choosing to not consider (skip) chunk $i^\prime$ rather than a later one is that $i^\prime$ is the closest to its deadline. Therefore, $i^\prime$ is not better candidate to the next quality level than any of the later ones.

In the second case of deadline/bandwidth violation, {\bf level-n}  backward algorithm decides to skip chunks up to $i^\prime$ since there is not enough bandwidth. As before, since equal number of chunks need to be skipped any way, skipping earlier ones is the best choice because it helps increasing the potential of getting later chunks at higher quality level.

Finally, we handle an inaccurate bandwidth estimation by setting lower buffer threshold, so if the buffer is running lower than this threshold, we reduce the level decision that was made by our Deadline and Buffer Aware Bin Packing Algorithm for the next chunk by 1 quality level (except if chunk is already at lowest quality). 

	
	
\begin{figure}[hbtp]
		%\vspace{-.6in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $B, X, C, deadline, Bm, bf,I_0$
				\STATE {\bf Output:} $t(i)$, $a(i)$, $e(j)$

   \STATE $ j=1$, $k=1$
    \WHILE {$j \leq deadline(C)$ and $k \leq max(I_0)$ (last chunk to fetch)}
	\STATE $i=I(k)$
          \STATE {\bf if }{$i=0$} {\bf then } $k=k+1$
            \IF{$j \leq deadline(i)$}
             \STATE {\bf if } {$(bf(j) = B_m)$} {\bf then }  $j=j+1$
                 \STATE $fetched=min(B(j), X(i))$
                \IF{$j$ is the first time chunk $i$ is fetched}
                 \STATE $t(i)=j$, $a(i)=fetched$ 
                    \ENDIF

                 \STATE $B(j)=B(j)-fetched$, $e(j)=B(j)$, $X(i)=X(i)-fetched$

                   \STATE {\bf if } {$X(i) > 0$} {\bf then }  $bf(j)=bf(j)+L$% and $j \geq t(i)$}
                  \STATE {\bf if } {$X(i)=0$} {\bf then } $k=k+1$

                   \STATE {\bf if } {$B(j)=0$} {\bf then } $j=j+1$
               \ELSE
                \STATE $k=k+1$
            \ENDIF

   \ENDWHILE


				\end{algorithmic}
				\caption{{\bf Level-n} Forward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}


\begin{figure}
		%\vspace{-.6in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $B, X,X_0, C, L, deadline, B_m,bf,t,r,a,e$					\STATE {\bf Output:} $X(i)$, $I_n$
    \STATE {\bf Initilization:}
    \STATE $i=C$, $ j=deadline(C)$
     \WHILE {($j > 0$ and $i > 0$)}
        \IF{$j <= deadline(i)$}
        \STATE {\bf if} {$(bf(deadline(i)) = B_m)$} {\bf then } $i=i-1$
              % \STATE continue
%         \ENDIF

                \IF{$j$ is the first time to fetch chunk $i$ from back}
                		\IF{$(t(i)=0)$}
				\STATE $rem1=c(j)-c(1)+e(1)$, $rem2=rem1$
				%\STATE $rem2=rem1$
			\ELSE
			\STATE $rem2=c(j)-c(t(i))$, $rem1=rem2+e(t(i))+a(i)$
				
			\ENDIF
                		\IF{$(rem1 < X_n(i))$}
				\STATE {\bf if} {$(X(i) > 0)$} {\bf then} $X_n(i)=X(i)$ {\bf else } $i=i-1$
			 \ELSE
		        		
                			\IF{$(rem2 < X_n(i))$ and $rem1 \geq X_n(i))$}
                				\STATE $e(t(i))=e(t(i))+rem1-X_n$
				\ENDIF
			        \STATE $X(i)=X_n(i)$, $I_n \leftarrow I_n\cup i$
            		\ENDIF
          	\ENDIF
	
            \STATE $fetched=min(B(j), X_n(i))$ 
            \STATE $B(j)=B(j)-fetched$, $X_n(i)=X_n(i)-fetched$
            \STATE  {\bf if} {$(X_n(i) > 0)$} {\bf then } $bf(j)=bf(j)+L$
            	
            \STATE {\bf if } {$(X_n(i)=0)$} {\bf then } $i=i-1$
	
	   \STATE {\bf if } {$(B(j)=0)$} {\bf then }  $j=j-1$            	
            \ELSE
           \STATE $j=j-1$
        \ENDIF
\ENDWHILE
				\end{algorithmic}
				\caption{{\bf Level-n} Backward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}






==> emulation.tex <==


\subsection{Emulation over TCP/IP Networks}
\label{sec:eval_emulation}

\begin{figure}
 \vspace{-.2in}
\includegraphics[trim=1.2in 0in 1.4in .1in, clip, width=0.38\textwidth, height=3in]{sigmetric_results/simVsemuV2.eps}
 \vspace{-.3in}	
  \caption{Emulation vs simulation: (a) playback bitrate over time, (b) chunk quality distribution. \feng{Reduce the space between the two plots. Remove ``Empirical CDF''.}}
  \label{fig:emu}
   \vspace{-.3in}
\end{figure}

To complement our simulation results, we have built an emulation testbed using C++ (about 1000 LoC) on Linux.
The testbed consists of a client and server. All streaming logic described in~\S\ref{sec:alg} is implemented on the client side, which fetches synthetic chunks from the server over a persistent TCP connection. We deploy our emulation testbed between a commodity laptop and a server inter-connected using high-speed Ethernet (1Gbps link and 1ms RTT).
We use \texttt{Dummynet}~\cite{dummynet} on the client side to replay a bandwidth profile by dynamically changing the available bandwidth every one second.
We also use the Linux \texttt{tc} tool to inject additional latency between the client and server.

We next run the emulation experiment using a 15-minute trace that we collected on LTE network, and since the bandwidth of the trace is high, we used SVC the following SVC rates, $1,5Mbps$ (BL), $2.75Mbps$ (EL 1), $4.8Mbps$ (EL 2), $7.8Mbps$ (EL 3) ~\cite{SVCDataset} . We configure the end-to-end RTT to be 30ms, which roughly corresponds to the last-mile latency in today's LTE networks. Meanwhile, we run the same bandwidth trace under identical settings using the simulation approach. Fig~\ref{fig:emu}-a compares the simulation and emulation results in terms of the qualities of fetched chunks, and Fig~\ref{fig:emu}-b compares the chunk quality distribution. As shown, the simulation and emulation results well cross-validate each other. Their slight difference in Fig~\ref{fig:emu}-a is mainly caused by the TCP behavior (\eg slow start after idle) that may underutilize the available bandwidth. We also increase the end-to-end RTT to 60ms, and observe qualitatively similar results except that the impact of TCP, which is not considered by our simulation, is higher.




% \section{Real time algorithm\\ emulation and results}
% \subsection{offline}
% To further investigate how our algorithm does in real network scenario and how results that we have using simulator is accurate in real scenarios, we built an emulator in C++. The emulator is described as follow:
%
% We start with comparing the offline case of the emulator with the corresponding one in the simulator. In this case, we assume a short video of 2 minutes length, full non causal knowledge of the bandwidth profile. The optimizer finds the optimal fetching policy offline and passes the policy to the emulator fetcher to start downloading the frames according to the pre-decided quality.
%
% \begin{figure *}
% \centering
% \epsfig{file=figures/emu1.pdf, height=2in, width=3in}
% \epsfig{file=figures/sim_vs_emu1.pdf, height=2in, width=3in}
% \caption{moderate average bandwidth (a) simulator fetching and playback, (b) emulator fetching and playback }
% \label{fig:simVsEm1}
% \end{figure *}
%
% \begin{figure *}
% \centering
% \epsfig{file=figures/emu3.pdf, height=2in, width=3in}
% \epsfig{file=figures/sim_vs_emu3.pdf, height=2in, width=3in}
% \caption{ Low average bandwidth (a) simulator fetching and playback, (b) emulator fetching and playback }
% \label{fig:simVsEm1}
% \end{figure *}
%
% \subsection{online}


==> noskipproof.tex <==
\section{Proof of Lemma \ref{lemma: noSkipLemma1}}\label{apdx:lemma1Noskip}

We note that for any feasible algorithm, we can convert to an in-order feasible streaming algorithm with the same time of receiving the last chunk. For an in-order streaming algorithm, the proposed base layer forward algorithm is a greedy algorithm that only adds to the deadline if the chunk cannot be downloaded in time due to not enough bandwidth. Further, the algorithm fetches all the chunks at only base layer quality which would have the lowest possible fetching times. Due to this greedy nature, no other algorithm can fetch all the chunks before those obtained by this greedy algorithm. 

\section{Proof of Theorem \ref{thm:noskip}}\label{apdx:lthem2Proof}

{From Lemma~\ref{lemma: noSkipLemma1}, we see that No-Skip forward algorithm finds the minimum stall duration such that all chunks can be fetched at least at base layer quality. However, after finding the minimum stall duration, the remaining part of the algorithm is similar to the skip based streaming problem since skips are allowed for enhancement layers. The No-Skip based streaming is a special case of the skip based streaming in which the chunk deadlines are chosen such that there are no base layers skips. Therefore, the rest of the proof follows the same lines as the proof of Theorem~\ref{theorem: theorem1} in Section~\ref{skipalgo}.}

==> proofsV3.tex <==
\section{Proof of Lemma \ref{lemma: noSkipLemma1}}\label{apdx:lemma1Noskip}

We note that for any feasible algorithm, we can convert to an in-order feasible streaming algorithm with the same time of receiving the last chunk. For an in-order streaming algorithm, the proposed Level-0 forward algorithm is a greedy algorithm that only adds to the deadline of a chunk if the chunk cannot be downloaded in time due to not enough bandwidth. Further, the algorithm fetches all the chunks at the lowest quality level which would have the lowest possible fetching times. Due to this greedy nature, no other algorithm can fetch all the chunks before those obtained by this greedy algorithm. 

\section{Proof of Lemma \ref{lem:skip:beta1}}\label{apdx:skip:beta1}

We first note that using the backward algorithm, a chunk $i_s$ is skipped from the $n$-th quality level decision in three scenarios, which are described as follows.


\noindent {\bf Case 1: } If the chunk $i_s$ is not a candidate to the $(n-1)$th level. This chunk should not be considered for the $n$-th level due to constraint (\ref{equ:c2eq1}).

\noindent {\bf Case 2: } The residual bandwidth in $(t(i_s)\quad to \quad deadline(i_s))$, ignoring the bandwidth used to fetch up to ($n-1$)-th levels of chunks less than $i_s$ (lower layer decisions) and the bandwidth used to fetch up to $n$-th level of chunks greater than $i_s$ (current layer decisions for later chunks) is not enough to fetch chunk $i_s$ at the $n$-th quality level. Mathematically, let's define $\pi_{prior}$ as what is reserved to fetch up to $(n-1)$-th level of chunks $< i_s$, and $\pi_{later}$ as what is reserved to fetch up to $n$-th level of chunks $> i_s$. Since decision of the current level starts from back, then chunk $i_s$ is skipped at the $n$-th level when: %{\bf Anis, have equation more precisely - $x$ is only for last layer decision - you have to take new layer decisions for future chunks. }

%Secondly, when after removing whatever reserved to fetch lower layers of prior chunks and up to $n$th layer of later chunks, the bandwidth from the lower to the higher deadline of chunks $i_s$ $(t(i_s)\quad to \quad deadline(i_s))$ is not enough to fetch chunk $i_s$ at $n$th layer quality. Mathematically:
\begin{equation}
\sum_{j=t(i_s)}^{deadline(i_s)}B(j) - \pi_{prior} -\pi_{later} < X_{n-1}+Y_{n}
%\sum_{i^\prime \neq i_s}\sum_{j=t(i_s+1)}^{deadline(i_s)}(x(i^\prime,j)) < X_{n-1}+Y_{n}
 \end{equation}
%Where, $X_{n-1}=\sum_{n=0}^{n-1}Y_n$, and $x(i^\prime,j)$ is the fetching policy of every chunk $i^\prime \neq i_s$.

\noindent {\bf Case 3: } If the $Y_n$ of chunk $i_s$ is obtained, the buffer constraint becomes violated. {\em i.e.}, when chunks $i_s$ to $i_e$ (excluding the skipped chunks in between) need to be in the buffer at a certain time in order not to skip $Y_n$ of chunk $i_s$, but their length is longer than the buffer duration. Mathematically there is a segment of chunks, $I=\{i_s,.....,i_e\}$  with length $N=i_e-i_s+1- \sum_{i_s}^{i_e} {\bf1}\{ Z_0(i)=0\} $, such that:
 \begin{equation}
N \cdot L > B_m
 \end{equation}
 %\end{enumerate}
 
 We note that the forward algorithm fetches chunks at the earliest possible time while the backward algorithm fetches chunks at the latest possible time. We will now show that the backward algorithm has no higher number of skips at any level (given previous level quality decisions) as compared to any other feasible algorithm. 
 
  
Any  skips which are due to Case 1 will be the same for any feasible algorithm. Thus, we do not consider skips that are of Case 1.  For the skip of Case 2 and Case 3, we first consider the last skip by our algorithm. We note that since the backward algorithm will fetch a $Y_n$ of any chunk if at all possible, if there is a skip at $i_s$, any algorithm will have a skip for a chunk $i\ge i_s$. Further note that skipping $Y_n$ of chunk $i_s$ as compared to $Y_n$ of chunk $i > i_s$ will allow for more bandwidth and buffer availability till deadline for the earlier chunks in the backward algorithm. Thus, if there is another skip using the backward algorithm, there must be another skip at or after the time of that skip in any other algorithm. Hence, we see that the number of skips in any feasible algorithm can be no less than the proposed algorithm. 


\section{Proof of Lemma \ref{lem:avoid_skips4}}\label{apdx:skip:betage1}

We note from Appendix \ref{apdx:skip:beta1} that for any skip of backward algorithm, there must be a skip or more for any other feasible algorithm. Further, since any feasible algorithm that has more number of skips can't achieve higher objective, we consider algorithms with a number of skips that is equal to what is achieved by the backward algorithm.

 In this case, we note from Appendix \ref{apdx:skip:beta1} that if the ordered set of skips for the backward algorithm are $i_1, i_2, \cdots, i_H$  and for any feasible algorithm are $j_1, j_2, \cdots, j_H$,  then $i_k\le j_k$ for all $k=1, \cdots, H$. Using this, and knowing that earlier skips will free up bandwidth that can be used to increase the quality of more chunks since it comes before the deadlines of more chunks than any other choice, we see that the result in the statement of the Lemma holds. 

%Scenario 2: The other feasible algorithm has more number of skips. However, we know when 

%Let the ordered set of skips for the backward algorithm are $i_1, i_2, \cdots, i_H$  and for any feasible algorithm are $j_1, j_2, \cdots, j_H, \cdots, j_{H+F}$. From the same arguments as in Appendix \ref{apdx:skip:beta1}, we see that there is a subsequence of $j_1, j_2, \cdots, j_H, \cdots, j_{H+F}$ given by $t_1, \cdots, t_H$ such that $i_k\le t_k$ for all $k=1, \cdots, H$ which proves the statement of the Lemma.  








\section{Proof of Theorem \ref{theorem: theorem1}}\label{apdx:them1}
From Lemma \ref{apdx:lemma1Noskip}, we know that the proposed algorithm finds the optimal deadline of every chunk such that all chunks can at least be fetched at the $0$-th quality level. Therefore $Y_0$ of every chunk can be fetched, and the stall duration is at its minimum.  We note that the conditions, $0<\beta < 1$ and  (\ref{basic_gamma_1}) depict the  priority of horizontal scanning over vertical scanning. It tells that fetching the $Y_1$ of one chunk achieves higher objective than fetching $Y_{2,\cdots , N}$ of all the chunks. Therefore, if $\beta$ satisfy the stated condition, the sequential scanning among different levels starting from the $0$-th level can show the optimality of the proposed algorithm. %we only need to show that sequential scanning starting from base layer up to the highest enhancement layer guarantee the optimality of the solution.

%{\bf Anis, Lemma numbers cannot be hard coded - Please use label and ref. }

{Lemmas~\ref{lem:skip:beta1} and \ref{lem:avoid_skips4} prove that running the backward algorithm for the $n$th level given lower and upper deadlines of every chunk achieves the optimal objective for the $n$th level and maximize resources for higher levels. Applying this to the $1^{st}$ level yields the optimal number of $1^{st}$ level skips and the maximum available bandwidth to every chunk that is candidate to the $n$-th level.}

{According to proposition \ref{noSkipPro}, running the forward algorithm for sizes decided by the backward algorithm on the $1^{st}$ quality level would fetch chunks at their earliest. Therefore, the lower deadline of every chunk such that all chunks are fetched according to the $1^{st}$ quality level is found by the forward algorithm.}

{Given the optimal lower deadlines of all chunks, running the backward algorithm on $2^{nd}$ quality level would produce the optimal $2^{nd}$ quality level decision without violating lower level decisions.  Scanning sequentially up to $M$th level would yield the optimal decisions of levels $0$ to $M$, and that concludes the proof.}


